Structural Tractability Frontiers for Metric Repair

Given a graph $G$ labeled with positive distances on each edge, what is the fewest number of edge distances that must be modified for $G$ to become a metric? It is known that this metric repair problem is $\mathrm{NP}$-hard on general graphs, with prior work focusing on approximations and fixed-parameter tractability with respect to properties of the input distance function. In this paper, we ask what structural properties of the graph itself make metric repair tractable. On the positive side, we give pseudo-polynomial time algorithms for series-parallel graphs, and by generalization, graphs of bounded treewidth. An immediate consequence of this result is a new algorithm for the length-bounded multicut problem, with a parameterized runtime bound in terms of the treewidth of a modestly augmented graph. Surprisingly, pseudo-polynomial time turns out to be the best one can hope for: We complement our algorithm with a proof that metric repair is weakly $\mathrm{NP}$-hard even on graphs of pathwidth at most six. We also prove that planarity does not help either, as the problem remains strongly $\mathrm{NP}$-hard even on grid graphs.

==> DBillustrate.tex <==
% !TEX root = GridGraphs.tex


\begin{figure}[t]
\centering
\begin{tikzpicture}[
    scale=1.15,
    every node/.style={font=\small},
    bagv/.style={circle, draw=red!70!black, fill=red!12, thick, inner sep=1.7pt},
    procv/.style={circle, draw=blue!60!black, fill=blue!8, inner sep=1.4pt},
    restv/.style={circle, draw=gray!70, fill=gray!12, inner sep=1.4pt},
    lightedge/.style={thick, blue!70!black},
    heavyedge/.style={thick, orange!85!black},
    restedge/.style={thick, gray!65},
    bagedge/.style={thick, red!55!black, dashed},
    edgelab/.style={fill=white, inner sep=1pt, font=\scriptsize},
    note/.style={align=left, font=\small}
]

% =========================================================
% Outerplanar embedding: all vertices on the outer face
% cyclic order: a, x, b, u, c, z
% =========================================================

\node[bagv, label=above:\(a\)]       (a) at (90:2.35) {};
\node[procv, label=above left:\(x\)] (x) at (150:2.35) {};
\node[bagv, label=left:\(b\)]        (b) at (210:2.35) {};
\node[restv, label=below:\(u\)]      (u) at (270:2.35) {};
\node[bagv, label=right:\(c\)]       (c) at (330:2.35) {};
\node[procv, label=above right:\(z\)](z) at (30:2.35) {};

% Optional outer-face guide
\draw[gray!25, dashed] (a)--(x)--(b)--(u)--(c)--(z)--(a);

% =========================================================
% Bag triangle: shown dashed as the separator bag
% =========================================================
\draw[bagedge] (a)--(b);
\draw[bagedge] (b)--(c);
\draw[bagedge] (c)--(a);

% =========================================================
% Processed subgraph G_t
% Choose labels so binary signature is easy:
% a-x-b is light-light => 0 in Pi(a,b)
% b-c is heavy => 1 in Pi(b,c)
% a-z-c is heavy-heavy => 2 in Pi(a,c)
% =========================================================

\draw[lightedge] (a)--(x) node[midway, above left, edgelab] {\(0\)};
\draw[lightedge] (x)--(b) node[midway, left, edgelab] {\(0\)};

\draw[heavyedge] (b)--(c) node[midway, below, edgelab] {\(1\)};

\draw[heavyedge] (a)--(z) node[midway, above right, edgelab] {\(1\)};
\draw[heavyedge] (z)--(c) node[midway, right, edgelab] {\(1\)};

% =========================================================
% Unprocessed remainder: one gray ear attached to b,c
% =========================================================

\draw[restedge] (b)--(u)--(c);

% =========================================================
% Labels
% =========================================================

\node[note, blue!70!black] at (-3.7,2.25)
{\(\boldsymbol{G_t}\): processed edges};

\node[note, blue!70!black] at (-4.0,0.0)
{\(0 \in \Pi(a,b)\) via \(axb\)\\
\(1 \in \Pi(b,c)\) via \(bc\)\\
\(2 \in \Pi(a,c)\) via \(azc\)};

\node[note, gray!70!black] at (-3.65,-2.0)
{unprocessed remainder\\
still to be handled by the DP};

\node[note, red!70!black] at (4.15,-0.25)
{\(B_t=\{a,b,c\}\)\\
the boundary bag};

% Small legend
\draw[lightedge] (2.7,1.75)--(3.35,1.75);
\node[right] at (3.35,1.75) {\scriptsize light edge};

\draw[heavyedge] (2.7,1.35)--(3.35,1.35);
\node[right] at (3.35,1.35) {\scriptsize heavy edge};

\draw[restedge] (2.7,0.95)--(3.35,0.95);
\node[right] at (3.35,0.95) {\scriptsize unprocessed edge};

\draw[bagedge] (2.7,0.55)--(3.35,0.55);
\node[right] at (3.35,0.55) {\scriptsize bag chord};

\end{tikzpicture}
\caption{An outerplanar DP snapshot.  All vertices lie on the outer face, and the graph is drawn without crossings.  The bag \(B_t=\{a,b,c\}\) is shown by dashed chords.  The processed subgraph \(G_t\) is represented by the colored processed edges; the remaining gray ear is unprocessed.}
\label{fig:outerplanar-dp-snapshot}
\end{figure}

\begin{figure}[t]
\centering
\begin{tikzpicture}[
    scale=1,
    every node/.style={font=\small},
    bagv/.style={circle, draw=red!70!black, fill=red!12, thick, inner sep=1.6pt},
    intv/.style={circle, draw=blue!60!black, fill=blue!8, inner sep=1.4pt},
    lightedge/.style={thick, blue!70!black},
    heavyedge/.style={thick, orange!85!black},
    sigbox/.style={draw, rounded corners, fill=gray!5, inner sep=6pt, align=left},
    joinbox/.style={draw, rounded corners, fill=gray!12, inner sep=6pt, align=center},
    lab/.style={font=\scriptsize, fill=white, inner sep=1pt}
]

% =========================================================
% Left child G1
% =========================================================
\begin{scope}[xshift=0cm,yshift=0cm]
    % bag vertices
    \node[bagv, label=above:\(a\)] (a1) at (0,1.8) {};
    \node[bagv, label=below left:\(b\)] (b1) at (-1.4,-0.8) {};
    \node[bagv, label=below right:\(c\)] (c1) at (1.4,-0.8) {};

    % internal vertex
    \node[intv, label=left:\(x\)] (x1) at (-1.9,0.7) {};

    % edges
    \draw[lightedge] (a1)--(x1) node[midway, above left, lab] {\(0\)};
    \draw[lightedge] (x1)--(b1) node[midway, left, lab] {\(0\)};
    \draw[heavyedge] (b1)--(c1) node[midway, below, lab] {\(1\)};

    % title
    \node[above=0.45cm of a1] {\(\boldsymbol{G_1}\)};

    % signature box
    \node[sigbox, below=1.1cm of $(b1)!0.5!(c1)$, anchor=north] (sig1) {
    \begin{minipage}{5.1cm}
    \[
    \Pi_1(a,b)=\{0\},\,
    \Pi_1(b,c)=\{1\},
    \]
    \[
    \Pi_1(a,c)=\{1\}.
    \]
    \scriptsize The value \(1\in\Pi_1(a,c)\) comes from closure:
    \(0\in\Pi_1(a,b)\) and \(1\in\Pi_1(b,c)\).
    \end{minipage}
    };
\end{scope}

% =========================================================
% Right child G2
% =========================================================
\begin{scope}[xshift=8.2cm,yshift=0cm]
    % bag vertices
    \node[bagv, label=above:\(a\)] (a2) at (0,1.8) {};
    \node[bagv, label=below left:\(b\)] (b2) at (-1.4,-0.8) {};
    \node[bagv, label=below right:\(c\)] (c2) at (1.4,-0.8) {};

    % internal vertex
    \node[intv, label=right:\(z\)] (z2) at (1.9,0.7) {};

    % edges
    \draw[heavyedge] (a2)--(z2) node[midway, above right, lab] {\(1\)};
    \draw[heavyedge] (z2)--(c2) node[midway, right, lab] {\(1\)};

    % title
    \node[above=0.45cm of a2] {\(\boldsymbol{G_2}\)};

    % signature box
    \node[sigbox, below=1.1cm of $(b2)!0.5!(c2)$, anchor=north] (sig2) {
    \begin{minipage}{4.1cm}
    \[
    \Pi_2(a,b)=\emptyset,\,
    \Pi_2(b,c)=\emptyset,
    \]
    \[
    \Pi_2(a,c)=\{2\}.
    \]
    \scriptsize The only boundary-to-boundary path is
    \(a\to z\to c\), which has two heavy edges.
    \end{minipage}
    };
\end{scope}

% =========================================================
% Join node and merged signature
% =========================================================
\node[joinbox] (join) at (4.1,-5.75) {\(\textsc{Join at } B_t=\{a,b,c\}\)};

% =========================================================
% Join arrows
% =========================================================
\coordinate (joinleft)  at (join.west);
\coordinate (joinright) at (join.east);

\draw[-{Latex[length=2mm]}, thick]
    (sig1.south) -- ++(0,-0.45) -| (joinleft);

\draw[-{Latex[length=2mm]}, thick]
    (sig2.south) -- ++(0,-0.45) -| (joinright);



\node[sigbox, below=0.55cm of join, anchor=north] (merged) {
\begin{minipage}{9.6cm}
\textbf{Validity test.}
The join is allowed if there is no boundary pair \(u,v\) and no
\(p\in\Pi_1(u,v)\), \(q\in\Pi_2(u,v)\) with \(p+q=1\).

In this example, the only pair that appears in both children is \((a,c)\), with
\[
1\in \Pi_1(a,c)\quad 2\in \Pi_2(a,c).
\]
Since \(1+2\neq 1\), the join is valid.

\medskip

\textbf{Merged signature.}
Taking the union and then closing under concatenation gives
\[
\Pi(a,b)=\{0\},\,
\Pi(b,c)=\{1\},\,
\Pi(a,c)=\{1,2\}.
\]
\end{minipage}
};

\end{tikzpicture}
\caption{A join step in the binary outerplanar dynamic program.  The two child subgraphs \(G_1\) and \(G_2\) have the same boundary bag \(B_t=\{a,b,c\}\).  Their signatures are merged provided no pair of boundary paths creates a bad cycle.}
\label{fig:outerplanar-join}
\end{figure}

==> IOMR_ladder.tex <==
% !TEX root = GridGraphs.tex
\subsection{Pseudo-polynomial time algorithm for IOMR on ladders}

We turn now to the general ladder graph, where the initial edge lengths are arbitrary positive integers and repairs must also assign positive integer lengths.  We give a dynamic program that computes an optimal repair in pseudo-polynomial time.  The key point is that for a ladder, the boundary between the processed and unprocessed portions always consists of exactly two vertices, so the dynamic-programming state collapses to a single
scalar.

Assume all initial edge lengths are positive integers and all repaired edge lengths must lie in $\{1,2,\dots,W\}$. For a repaired prefix \(L^{\le i}\), define the boundary distance
\[
\delta_x(i)\defeq \dist_{x,L^{\le i}}(u_i,v_i).
\]
Because all repaired lengths lie in \(\{1,\dots,W\}\), every boundary distance satisfies $\delta_x(i)\in\{1,\dots,W\}$.

Because of the structure of the ladder, the validity of a repaired prefix \(L^{\le i}\) depends only on the repaired lengths of the three edges in the top square \(Q_i\) and the boundary distance \(\delta_x(i-1)\).  This is captured by the following lemma which provides the inductive step of the dynamic program.
\begin{lemma}[One-square extension]
\label{lem:one-square-extension}
Let \(x\) be a feasible repair of the prefix \(L^{\le i-1}\), and set
$\delta=\dist_{x,L^{\le i-1}}(u_{i-1},v_{i-1})$.
Suppose we extend \(x\) to the next square \(Q_i\) by assigning repaired lengths
\[
    a=x(\ell_i)\ge w(\ell_i),\qquad b=x(r_i)\ge w(r_i),\qquad t=x(e_i)\ge w(e_i).
\]
Then the extended repair is feasible on \(L^{\le i}\) if and only if the following three inequalities hold:
\[
    t\le a+\delta+b,\qquad
    a\le t+\delta+b,\qquad
    b\le t+\delta+a.
\]
Moreover, whenever they hold $\dist_{x,L^{\le i}}(u_i,v_i)=t$.
\end{lemma}
\begin{proof}
It suffices to check the three edges $\ell_i$, $r_i$, and $e_i$ that are introduced when we extend from $L^{\le i-1}$ to $L^{\le i}$, since the validity of all other edges is unaffected by the extension. 

For the top rung \(e_i\), the alternative path from \(u_i\) to \(v_i\) goes down \(\ell_i\), across
the old prefix from \(u_{i-1}\) to \(v_{i-1}\), and up \(r_i\).  Its length is $a+\delta+b$ and hence \(e_i\) is valid iff $t\le a+\delta+b$. Similarly, for the other edges.

Finally, in \(L^{\le i}\), the two relevant \(u_i\)-to-\(v_i\) routes are the direct rung \(e_i\),
of length \(t\), and the detour through the old prefix, of length \(a+\delta+b\).  Since $t\le a+\delta+b$, the direct rung is shortest.  Therefore, $\dist_{x,L^{\le i}}(u_i,v_i)=t$.
\end{proof}

For \(i\in\{0,\ldots,m\}\) and \(t\in\{1,\ldots,W\}\), let \(A_i(t)\) be the minimum number of
modified edges in a feasible repair of \(L^{\le i}\) whose boundary distance is \(t\); that is,
\(A_i(t)\) is the minimum cost over all repairs \(x\) of \(L^{\le i}\) such that
\(\dist_{x,L^{\le i}}(u_i,v_i)=t\).  If no such repair exists, set \(A_i(t)=+\infty\).

The base case is
\[
A_0(t)=
\begin{cases}
0, & t=w(e_0),\\
1, & w(e_0)<t\le W,\\
+\infty, & \text{otherwise.}
\end{cases}
\]

For \(i=1,\ldots,m\), define the local transition cost \(C_i(\delta,t)\) as follows.  Given an old
boundary distance \(\delta\) and a desired new boundary distance \(t\), \(C_i(\delta,t)\) is the
minimum number of modified edges among the three new edges \(\ell_i,r_i,e_i\) needed to extend the
prefix across square \(Q_i\).  Equivalently, \(C_i(\delta,t)\) is the minimum of
\[
\mathbf{1}[a>w(\ell_i)]+\mathbf{1}[b>w(r_i)]+\mathbf{1}[t>w(e_i)]
\]
over integers \(a,b\in\{1,\ldots,W\}\) satisfying \(a\ge w(\ell_i)\), \(b\ge w(r_i)\),
\(t\ge w(e_i)\), and
\[
t\le a+\delta+b,\qquad
a\le t+\delta+b,\qquad
b\le t+\delta+a.
\]
If no such \(a,b\) exist, set \(C_i(\delta,t)=+\infty\).

The recurrence is
\[
A_i(t)=
\min_{\delta\in\{1,\ldots,W\}}
\left\{
A_{i-1}(\delta)+C_i(\delta,t)
\right\}.
\]

Finally, the optimum repair cost for the full ladder is
\[
\mathrm{OPT}(L_m)=\min_{t\in\{1,\ldots,W\}} A_m(t).
\]

We can thus conclude the following.
\begin{theorem}
Bounded-integer IOMR on a ladder \(L_m\), with repaired edge lengths restricted to
\(\{1,\ldots,W\}\), can be solved exactly in pseudo-polynomial time.
More precisely, using the dynamic program above, the optimum repair cost is computed in
\(O(mW^2)\) time after precomputing the local transition costs \(C_i(\delta,t)\), or in
\(O(mW^3)\) time with direct enumeration of the local transitions.
\end{theorem}

Since the running time is polynomial in the numeric bound \(W\), the algorithm is pseudo-polynomial.


==> OPgraphexample.tex <==
% !TEX root = GridGraphs.tex
\begin{figure}[ht]
\centering
\begin{tikzpicture}[scale=1.05, every node/.style={font=\small}]

% =====================================
% Outerplanar graph
% =====================================
\begin{scope}[xshift=0cm]

    % vertices on a symmetric heptagon
    \node[circle, draw, inner sep=1.5pt] (v1) at (90:2.4) {$1$};
    \node[circle, draw, inner sep=1.5pt] (v2) at (38.57:2.4) {$2$};
    \node[circle, draw, inner sep=1.5pt] (v3) at (-12.86:2.4) {$3$};
    \node[circle, draw, inner sep=1.5pt] (v4) at (-64.29:2.4) {$4$};
    \node[circle, draw, inner sep=1.5pt] (v5) at (-115.71:2.4) {$5$};
    \node[circle, draw, inner sep=1.5pt] (v6) at (-167.14:2.4) {$6$};
    \node[circle, draw, inner sep=1.5pt] (v7) at (141.43:2.4) {$7$};

    % outer cycle
    \draw[thick] (v1)--(v2)--(v3)--(v4)--(v5)--(v6)--(v7)--(v1);

    % chords
    \draw[thick] (v1)--(v3);
    \draw[thick] (v3)--(v5);
    \draw[thick] (v5)--(v7);

    % title
    \node[above=0.75cm of v1] {\textbf{Example graph \(G\)}};

\end{scope}

% =====================================
% Tree decomposition
% =====================================
\begin{scope}[xshift=7.6cm]

    % root
    \node[draw, rounded corners, minimum width=3.45cm, minimum height=0.95cm] (t2) at (0,2.2)
        {\(t_2:\; B_{t_2}=\{1,3,5\}\)};

    % second layer
    \node[draw, rounded corners, minimum width=3.45cm, minimum height=0.95cm] (t1) at (-3.2,0.7)
        {\(t_1:\; B_{t_1}=\{1,2,3\}\)};
    \node[draw, rounded corners, minimum width=3.45cm, minimum height=0.95cm] (t3) at (0,0.7)
        {\(t_3:\; B_{t_3}=\{3,4,5\}\)};
    \node[draw, rounded corners, minimum width=3.45cm, minimum height=0.95cm] (t4) at (3.2,0.7)
        {\(t_4:\; B_{t_4}=\{1,5,7\}\)};

    % third layer
    \node[draw, rounded corners, minimum width=3.45cm, minimum height=0.95cm] (t5) at (3.2,-0.9)
        {\(t_5:\; B_{t_5}=\{5,6,7\}\)};

    % tree edges
    \draw[thick] (t2)--(t1);
    \draw[thick] (t2)--(t3);
    \draw[thick] (t2)--(t4);
    \draw[thick] (t4)--(t5);

    % title
    \node[above=0.75cm of t2] {\textbf{Tree decomposition \(\mathcal T\)}};

\end{scope}

\end{tikzpicture}
\caption{An example outerplanar graph together with a labeled width-\(2\) tree decomposition.}
\label{fig:outerplanar-example}
\end{figure}





\begin{figure}[p]
\centering
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
    x=1.8cm, y=-1.1cm,
    bag/.style={
        draw,
        rounded corners,
        align=center,
        inner sep=2pt,
        minimum width=2.8cm,
        minimum height=0.78cm,
        font=\scriptsize
    },
    leafbag/.style={bag, fill=green!18},
    introvbag/.style={bag, fill=blue!14},
    forgetbag/.style={bag, fill=orange!22},
    introebag/.style={bag, fill=violet!18},
    joinbag/.style={bag, fill=gray!18}
]

% =========================================================
% Legend
% =========================================================
\node[leafbag]   (L1) at (-8.7,0.0) {leaf};
\node[introvbag] (L2) at (-6.6,0.0) {introduce vertex};
\node[forgetbag] (L3) at (-3.8,0.0) {forget vertex};
\node[introebag] (L4) at (-1.0,0.0) {introduce edge};
\node[joinbag]   (L5) at (1.5,0.0) {join};

% =========================================================
% Root chain
% =========================================================
\node[forgetbag] (r0) at (0,1.8) {\(r_0:\ \emptyset\)\\[-1mm]\tiny forget \(5\)};
\node[forgetbag] (r1) at (0,3.1) {\(r_1:\ \{5\}\)\\[-1mm]\tiny forget \(1\)};
\node[forgetbag] (r2) at (0,4.4) {\(r_2:\ \{1,5\}\)\\[-1mm]\tiny forget \(3\)};
\node[joinbag]   (J2) at (0,5.9) {\(J_2:\ \{1,3,5\}\)\\[-1mm]\tiny join};

\draw (r0)--(r1)--(r2)--(J2);

% =========================================================
% Children of J2
% =========================================================
\node[joinbag]   (J1) at (-4.2,7.4) {\(J_1:\ \{1,3,5\}\)\\[-1mm]\tiny join};
\node[introvbag] (c0) at (4.2,7.4) {\(c:\ \{1,3,5\}\)\\[-1mm]\tiny introduce \(3\)};

\draw (J2)--(J1);
\draw (J2)--(c0);

% =========================================================
% Children of J1
% =========================================================
\node[introvbag] (a0) at (-6.5,8.9) {\(a:\ \{1,3,5\}\)\\[-1mm]\tiny introduce \(5\)};
\node[introvbag] (b0) at (-1.9,8.9) {\(b:\ \{1,3,5\}\)\\[-1mm]\tiny introduce \(1\)};

\draw (J1)--(a0);
\draw (J1)--(b0);

% =========================================================
% Branch A
% =========================================================
\node[forgetbag] (a1) at (-6.5,10.2) {\(\{1,3\}\)\\[-1mm]\tiny forget \(2\)};
\node[introebag] (a2) at (-6.5,11.5) {\(\{1,2,3\}\)\\[-1mm]\tiny intro \(13\)};
\node[introebag] (a3) at (-6.5,12.8) {\(\{1,2,3\}\)\\[-1mm]\tiny intro \(23\)};
\node[introebag] (a4) at (-6.5,14.1) {\(\{1,2,3\}\)\\[-1mm]\tiny intro \(12\)};
\node[introvbag] (a5) at (-6.5,15.4) {\(\{1,2,3\}\)\\[-1mm]\tiny introduce \(2\)};
\node[introvbag] (a6) at (-6.5,16.7) {\(\{1,3\}\)\\[-1mm]\tiny introduce \(3\)};
\node[introvbag] (a7) at (-6.5,18.0) {\(\{1\}\)\\[-1mm]\tiny introduce \(1\)};
\node[leafbag]   (a8) at (-6.5,19.3) {\(\emptyset\)};

\draw (a0)--(a1)--(a2)--(a3)--(a4)--(a5)--(a6)--(a7)--(a8);

% =========================================================
% Branch B
% =========================================================
\node[forgetbag] (b1) at (-1.9,10.2) {\(\{3,5\}\)\\[-1mm]\tiny forget \(4\)};
\node[introebag] (b2) at (-1.9,11.5) {\(\{3,4,5\}\)\\[-1mm]\tiny intro \(35\)};
\node[introebag] (b3) at (-1.9,12.8) {\(\{3,4,5\}\)\\[-1mm]\tiny intro \(45\)};
\node[introebag] (b4) at (-1.9,14.1) {\(\{3,4,5\}\)\\[-1mm]\tiny intro \(34\)};
\node[introvbag] (b5) at (-1.9,15.4) {\(\{3,4,5\}\)\\[-1mm]\tiny introduce \(4\)};
\node[introvbag] (b6) at (-1.9,16.7) {\(\{3,5\}\)\\[-1mm]\tiny introduce \(5\)};
\node[introvbag] (b7) at (-1.9,18.0) {\(\{3\}\)\\[-1mm]\tiny introduce \(3\)};
\node[leafbag]   (b8) at (-1.9,19.3) {\(\emptyset\)};

\draw (b0)--(b1)--(b2)--(b3)--(b4)--(b5)--(b6)--(b7)--(b8);

% =========================================================
% Branch C
% =========================================================
\node[forgetbag] (c1) at (4.2,8.9) {\(\{1,5\}\)\\[-1mm]\tiny forget \(7\)};
\node[introebag] (c2) at (4.2,10.2) {\(\{1,5,7\}\)\\[-1mm]\tiny intro \(57\)};
\node[introebag] (c3) at (4.2,11.5) {\(\{1,5,7\}\)\\[-1mm]\tiny intro \(17\)};
\node[introvbag] (c4) at (4.2,12.8) {\(\{1,5,7\}\)\\[-1mm]\tiny introduce \(1\)};
\node[forgetbag] (c5) at (4.2,14.1) {\(\{5,7\}\)\\[-1mm]\tiny forget \(6\)};
\node[introebag] (c6) at (4.2,15.4) {\(\{5,6,7\}\)\\[-1mm]\tiny intro \(67\)};
\node[introebag] (c7) at (4.2,16.7) {\(\{5,6,7\}\)\\[-1mm]\tiny intro \(56\)};
\node[introvbag] (c8) at (4.2,18.0) {\(\{5,6,7\}\)\\[-1mm]\tiny introduce \(6\)};
\node[introvbag] (c9) at (4.2,19.3) {\(\{5,7\}\)\\[-1mm]\tiny introduce \(7\)};
\node[introvbag] (c10) at (4.2,20.6) {\(\{5\}\)\\[-1mm]\tiny introduce \(5\)};
\node[leafbag]   (c11) at (4.2,21.9) {\(\emptyset\)};

\draw (c0)--(c1)--(c2)--(c3)--(c4)--(c5)--(c6)--(c7)--(c8)--(c9)--(c10)--(c11);

\end{tikzpicture}%
}
\caption{A colored nice tree decomposition for the outerplanar graph on vertices \(1,\dots,7\) with outer-cycle edges \(12,23,34,45,56,67,71\) and chords \(13,35,57\).  Colors indicate node type: leaf, introduce-vertex, forget-vertex, introduce-edge, and join.}
\label{fig:nice-decomposition}
\end{figure}


==> ladder.tex <==
% ------------------------------------------------------------------
\section{IOMR on Ladder Graphs}
\label{sec:binary-ladder}
% ------------------------------------------------------------------

Let $G = (V, E)$ be an $m \times n$ planar grid graph, defined by a matrix of vertices $(x, y)$ for $0 \le x \le m$ and $0 \le y \le n$. A \emph{ladder graph} is the special case $m = 1$. Let $L_m$ denote the ladder with rungs
\[
    e_0,e_1,\ldots,e_m
\]
and rail edges
\[
    \ell_i=\{u_{i-1},u_i\},\qquad r_i=\{v_{i-1},v_i\},\qquad i=1,\ldots,m.
\]
The $i$th square is the $4$-cycle
\[
    Q_i=(e_{i-1},\ell_i,e_i,r_i).
\]


\subsection{Binary IOMR on ladders}

Every simple cycle in a ladder is a rectangle.  For $0\le j<k\le m$, let $R_{j,k}$ be the rectangle
bounded by the two rungs $e_j,e_k$ and the two rail paths between them.  Thus
\[
    H_w(R_{j,k})
    =w(e_j)+w(e_k)+\sum_{i=j+1}^{k}\bigl(w(\ell_i)+w(r_i)\bigr).
\]

\begin{lemma}[Local-global equivalence for binary ladders]
A binary labeling $w$ is metrically valid on $L_m$ if and only if
\[
    H_w(Q_i)\ne 1 \qquad \text{for every } i=1,\ldots,m.
\]
Equivalently, for ladders it is enough to repair fundamental squares with exactly one heavy edge.
\label{lem:binary-ladder-local-global}
\end{lemma}

\begin{proof}
The forward direction is immediate since every square is a cycle.

For the reverse direction, assume that every square satisfies $H_w(Q_i)\ne 1$.  Suppose for contradiction that
some rectangle $R_{j,k}$ has exactly one heavy edge.  Then
\[
    w(e_j)+w(e_k)+\sum_{i=j+1}^{k}\bigl(w(\ell_i)+w(r_i)\bigr)=1.
\]
All terms are nonnegative integers, so exactly one term in this sum is equal to $1$, and all the
others are equal to $0$.

First suppose the unique nonzero term is a rail contribution
\[
    w(\ell_p)+w(r_p)=1
\]
for some $p\in\{j+1,\ldots,k\}$.  Then $w(e_j)=w(e_k)=0$, and all other rail contributions in the
rectangle are $0$.  Whenever $w(\ell_i)+w(r_i)=0$, the square condition says
\[
    w(e_{i-1})+w(e_i)\ne 1,
\]
so adjacent rungs across that square have the same label.  Propagating from $e_j$ upward gives
$w(e_{p-1})=0$, and propagating from $e_k$ downward gives $w(e_p)=0$.  Hence
\[
    H_w(Q_p)=w(e_{p-1})+w(\ell_p)+w(r_p)+w(e_p)=0+1+0=1,
\]
contradicting the square condition.

It remains to consider the case in which the unique heavy edge of $R_{j,k}$ is one of the two
boundary rungs.  By symmetry, suppose $w(e_j)=1$.  Then $w(e_k)=0$, and all rail contributions
between levels $j$ and $k$ are $0$.  As above, each square condition forces adjacent rungs to have
the same label, so
\[
    w(e_j)=w(e_{j+1})=\cdots=w(e_k),
\]
contradicting $w(e_j)=1$ and $w(e_k)=0$.  The case in which $e_k$ is the unique heavy edge is
identical.  Therefore no rectangle has exactly one heavy edge, and since every simple cycle in a
ladder is a rectangle, $w$ is globally valid.
\end{proof}

By Lemma~\ref{lem:binary-ladder-local-global}, the global feasibility condition reduces to the
local constraints
\[
    w(e_{i-1})+w(\ell_i)+w(r_i)+w(e_i)\ne 1,
    \qquad i=1,\ldots,m.
\]
Thus, when processing the ladder from bottom to top, the only information that must be passed from
one square to the next is the final label of the current top rung.

For $i=0,1,\ldots,m$ and $s\in\{0,1\}$, define $\mathrm{DP}_i(s)$
to be the minimum number of upgrades in the prefix $L^{\le i}$ such that all squares $Q_1,\ldots,Q_i$ are valid and the final label of the top rung $e_i$ is $s$.  If no such repair exists, set $\mathrm{DP}_i(s)=\infty$.

For an edge \(e\) and a target label \(z\in\{0,1\}\), define the upgrade cost
\[
    c_e(z)
    :=
    \begin{cases}
        0, & z=w(e),\\
        1, & w(e)=0 \text{ and } z=1,\\
        \infty, & w(e)=1 \text{ and } z=0.
    \end{cases}
\]
Thus \(c_e(z)\) enforces the increase-only constraint.

For \(i=0,\ldots,m\) and \(s\in\{0,1\}\), let $D_i(s)$
denote the minimum number of upgrades needed to repair the prefix \(L^{\le i}\), subject to the
condition that the top rung \(e_i\) receives final label \(s\).

The base case is
\[
    D_0(s)=c_{e_0}(s),
    \qquad s\in\{0,1\}.
\]

For \(i=1,\ldots,m\), the recurrence is
\[
    D_i(t)
    =
    c_{e_i}(t)
    +
    \min_{\substack{s,a,b\in\{0,1\}\\ s+a+b+t\neq 1}}
    \left\{
        D_{i-1}(s)
        +
        c_{\ell_i}(a)
        +
        c_{r_i}(b)
    \right\},
    \qquad t\in\{0,1\}.
\]
The answer is
\[
    \operatorname{OPT}(L_m)=\min\{D_m(0),D_m(1)\}.
\]

We can thus conclude the following.
\begin{theorem}
\label{thm:binary-ladder-dp-correctness}
The dynamic program returns the optimum value of binary IOMR on $L_m$ in $O(m)$ time.
\end{theorem}

The local-global equivalence above is special to ladders.  In wider grids, forbidding bad
fundamental squares does not in general forbid all bad cycles.


==> preliminaries.tex <==
%% ====================================================================
\section{Definitions and Notation}
%% ====================================================================


\begin{definition}[Increase-Only Metric Repair (IOMR)]
Given a graph $G = (V, E)$ and initial edge weights $w: E \to \mathbb{R}_{>0}$, find a corrected weight function $x: E \to \mathbb{R}_{>0}$ such that $x(e) \ge w(e)$ for all $e \in E$, minimizing the number of modified edges $|\{e : x(e) > w(e)\}|$, subject to the metric cycle property: for every cycle $C$ and every edge $e \in C$,
\[
    x(e) \le \sum_{e' \in C \setminus \{e\}} x(e').
\]
\end{definition}

\begin{definition}[Binary IOMR]
The restriction of IOMR where the initial weights are drawn from $\{1, M\}$ with $M > |V|$, and the corrected weights must also lie in $\{1, M\}$. 
\end{definition}

As each edge is either light or heavy in Binary IOMR, we write $w(e) = 0$ for the light edge weight and $w(e) = 1$ for the heavy edge weight. The increase-only constraint says that an edge initially labeled $1$ must remain $1$, while an edge initially labeled $0$ may either remain $0$ or be upgraded to $1$.  Since the heavy length $M$ is larger than the length of every simple cycle, a binary labeling is metrically valid if and only if no simple cycle contains exactly one heavy edge.

For a binary labeling $w:E(L_m)\to\{0,1\}$ and a cycle $C$, write
\[
    H_w(C):=\sum_{e\in C}w(e)
\]
for the number of heavy edges on $C$.
